On the Accuracy of Equivalent Antenna Representations

The accuracy of two equivalent antenna representations, near-field sources and far-field sources, are evaluated for an antenna installed on a simplified platform in a series of case studies using different configurations of equivalent antenna representations. The accuracy is evaluated in terms of installed far-fields and surface currents on the platform. The results show large variations between configurations. The root-mean-square installed far-field error is 4.4% for the most accurate equivalent representation. When using far-field sources, the design parameters have a large influence of the achieved accuracy. There is also a varying accuracy depending on the type of numerical method used. Based on the results, some recommendations on the choice of sub-domain for the equivalent antenna representation are given. In industrial antenna applications, the accuracy in determining e.g. installed far-fields and antenna isolation on large platforms are critical. Equivalent representations can reduce the fine-detail complexity of antennas and thus give an efficient numerical descriptions to be used in large-scale simulations. The results in this paper can be used as a guideline by antenna designers or system engineers when using equivalent sources.

==> Comments.tex <==
\textcolor{blue}{
-- I \textit{IEEE Transaction on Electromagnetic Compatibility} brukar fullst\"{a}ndiga artiklar ha 8-9 sidor, och \textit{Letters} cirka 4 sidor. \\
-- Emphasize reliability and predictability!
}

%\textcolor{olive}{
%\subsection*{Lars kommentarer  (this heading and the comments will be removed)}
%-- fundera p\aa{} vilken m\aa{}lgrupp vi har, och v\"{a}lj grad av vad som ska f\"{o}rklaras, vad vet l\"{a}sarna och vad beh\"{o}ver vi f\"{o}rklara f\"{o}r att de inte k\"{a}nner till?\\
%Lars kommentarer:\\
%%-- N\"{a}r jag l\"{a}ser den nuvarande text glider vi fr\aa{}n allm\"{a}n simuleringskunskap (i introduktionen) till unders\"{o}k en specifik antenn, str\"{o}mmar, fj\"{a}rrf\"{a}lt r\"{o}rande sig mot koppling  mellan antenner. -- jag skulle fokusera tidigare p\aa{} det vi \"{a}r intresserade av, f\"{o}rklara varf\"{o}r. \\
%-- fundera p\aa{} utifr\aa{}n vilka resultat du r\"{a}knar med att uppn\aa{}, hur introduktionen knyter n\"{a}ra an till dessa och som presenterar det specifika omr\aa{}det/problem som vi \"{a}r intresserade av.  
%}
%
%\textcolor{olive}{
%\subsection*{Lars kommentarer  (this heading and the comments will be removed)}
%%  -- jag skulle fokusera mer p\aa{} noggrannhet som huvudtema (och mindre p\aa{} att simulera r\"{a}tt) 
%%\\
%% --  Orsaken som b\aa{}de du och Henrik har pratat om \"{a}r noggrannhet och tillf\"{o}rlitlighet, detta \"{a}r en av de underliggande orsakerna till manuskriptet. 
%%\\
%% -- omr\aa{}det source modeling \"{a}r ett genom antennhistoriskt stort omr\aa{}de med m\aa{}nga som har k\"{a}nt sig kallade att modellera allt ifr\aa{}n delta-gapet p\aa{} dipolen till m\aa{}nga andra typer av resultat (fr\aa{}n Hallen och fram\aa{}t). F\"{o}r att f\aa{} ett papper accepterat inom detta omr\aa{}de b\"{o}r man citera huvudpapper inom litteraturen, och tydligt prata om hur detta papper skiljer sig fr\aa{}n dessa. Att visa en medvetenhet av vad som gjorts och hur detta resultat kompletterar tidigare arbeten. 
%\textcolor{olive}{ -- att lyfta upp och f\"{o}rklara vilka utv\"{a}rderingsparametrar som \"{a}r viktiga och varf\"{o}r (\aa{}terkommer sedan i resultat/utv\"{a}rdering)}\\
%-- om vi fokuserar p\aa{} noggrannhet beh\"{o}ver vi j\"{a}mf\"{o}ra med andra program, eller f\"{o}rklara varf\"{o}r det inte \"{a}r m\"{o}jligt. Det finns en special-version p\aa{} EuCap (de senaste \aa{}ren inkl 2016) under Guy Vandenbosch och Francesca Mioc 'Application Track: EM Modelling and simulation', d\"{a}r de jobbat tillsammans med flera stora f\"{o}retag f\"{o}r att oberoende j\"{a}mf\"{o}ra simuleringar och m\"{a}ta flera olika parametrar av sm\aa{} antenner, horn antenner mm H\"{a}r finns en utveckling som visar p\aa{} h\"{o}gskalig kvalitets-j\"{a}mf\"{o}relse mellan olika l\"{o}sare och m\"{a}tningar. (\"{A}ven f\"{o}r fall som betraktats av alla software f\"{o}retag under flera \aa{}r verkar det som om simulering och m\"{a}tningar skiljer sig ordentligt, \"{a}ven om de anv\"{a}nder samma metod, ocks\aa{} n\"{a}r de anv\"{a}nder olika metoder) FEKO, ANSOFT, EFIELD, CST mfl.  En sak som var tydlig p\aa{} de b\"{a}ttre av dessa j\"{a}mf\"{o}relser var att spridningen mellan l\"{o}sare (anv\"{a}nda av softwaref\"{o}retagens experter) nu har mycket mindre spridning \"{a}n tidigare. \\
%-- att lyfta upp och f\"{o}rklara vilka utv\"{a}rderingsparametrar som \"{a}r viktiga och varf\"{o}r (\aa{}terkommer sedan i resultat/utv\"{a}rdering)\\
%-- det \"{a}r viktigt att tydligt positionera sig och f\"{o}rklara vad det \"{a}r som skiljer sig med detta papper -- nyckelbegrepp h\"{a}r \"{a}r applikationsrelaterade och dessa b\"{o}r betonas f\"{o}r att positionera sig, och varf\"{o}r detta \"{a}r sv\aa{}rare/intressantare/ \"{a}n tidigare typer av utv\"{a}rderingar. \\
%%-- varje bild beh\"{o}ver ett stycke i texten som reflekterar \"{o}ver vad vi ser i dessa figurer, och hur detta tolkas. 
%%\\
%-- i figurer kan det vara bra att ha en zoom p\aa{} ett 'intressant' omr\aa{}de\\
%-- f\"{o}rklara vad vi f\aa{}r f\"{o}r impact av skillnaden rent praktiskt. 
%   (\"{a}r vi ute efter uppskattning av variation, absolut noggranhet mot m\"{a}tningar, annat)\\
%-- Koppla applikationsrelaterat intresse till noggrannhet.
%}
%
% 

==> Simulations.tex <==
% !TeX spellcheck = en_GB
% !TeX root = Sources_main.tex
%
\section{Simulation Results} 
\label{sec:Results}
%

%\"{A}r detta en geometri som f\aa{}ngar det effekter som vi vill se?

